Multilayer occupancy grid for obstacle avoidance in an autonomous ground vehicle using RGB-D camera

This work describes the process of integrating a depth camera into the navigation system of a self-driving ground vehicle (SDV) and the implementation of a multilayer costmap that enhances the vehicle's obstacle identification process by expanding its two-dimensional field of view, based on 2D LIDAR, to a three-dimensional perception system using an RGB-D camera. This approach lays the foundation for a robust vision-based navigation and obstacle detection system. A theoretical review is presented and implementation results are discussed for future work.

==> src/Anexos/Anexos.tex <==
\onecolumn

\begin{appendices}
    \input{src/Anexos/Docker/Docker.tex}
    
\end{appendices}

\twocolumn

==> src/Anexos/Docker/Docker.tex <==
\section*{Anexo I: Dockerfile}\label{anexo:dockerfile}
    A continuación se muestra el Dockerfile utilizado:
    \lstinputlisting[style=yaml]{src/Anexos/Docker/dockerfile.yml}
\newpage
\section*{Anexo II: Docker-compose}
    A continuación se muestra el archivo docker-compose utilizado:
    \lstinputlisting[style=yaml]{src/Anexos/Docker/docker-compose.yml}


==> src/Arquitectura/Arquitectura_de_Sistema.tex <==
\section{Background}\label{sec:system_architecture}

This section presents the structure and functioning of specific components of the navigation system (\textit{nav\_stack}) that enable trajectory planning and execution based on data provided by the perception system. The study of the multilayer costmap, used in trajectory generation, is introduced. Finally, the concepts of the operating theory and optical properties of the RGB-D camera are also presented.

\subsection{Navigation System}\label{sec:nodos_nav_stack}

The autonomous navigation system is implemented using the \textit{move\_base} navigation package from ROS~\cite{move_base_ros_node}. It uses costmaps to represent information about the environment's occupancy by objects. This information is used by local and global planners (\textit{global\_planner} and \textit{local\_planner}) for safe trajectory planning and generation. In the context of ROS's autonomous navigation stack, there are two main levels of costmaps: the \textit{global\_costmap} and the \textit{local\_costmap} (see fig. \ref{fig:move_base_arq}).

\begin{figure}[htbp]
    \centering
    \includegraphics[width=\columnwidth]{src/Integración RealSense SDV/imgs_D435I/move_base_arq.png}
    \caption{Costmap under the navigation system architecture of the SDV~\cite{move_base_ros_node}.}\label{fig:move_base_arq}
\end{figure}

\textit{Global Costmap:}  
The global\_costmap aims to provide a high-level occupancy representation of the environment and is used for global route planning. This costmap is generated using both static and dynamic information. The former generally comes from previously created occupancy maps and represents the unchanging environment, such as stationary robots or walls. On the other hand, the dynamic information provides a real-time representation of the robot's environment, such as a moving person or another vehicle, and comes directly from the perception system.

\textit{Local Costmap:}  
The local\_costmap, in contrast, describes the immediate environment of the robot and is used for local navigation. For example, it identifies nearby and moving obstacles. This costmap is updated more frequently and also utilizes information provided by the perception system.

\textit{Occupancy Grid:}  
The main representation of the environment in the global and local costmaps is an occupancy grid. In this grid, each cell represents a region of the environment and has a value indicating the level of occupancy. Typically, a scale of discrete values is used, such as: 0 (free cell), indicating that the cell is unoccupied, or 100 (occupied cell), indicating the presence of an obstacle. This grid is what the trajectory planning system ultimately uses to generate safe routes for navigating the environment.
\subsection{Multilayer Costmap}\label{sec:costmap}

The overlay of the global and local costmaps is referred to as the Multilayer Costmap. The occupancy grid generated from this map integrates both global and local information. Figure \ref{fig:costmap_multilayer} shows a conceptual representation of this map, where each costmap, whether global or local, can originate from specific sensors, such as LiDAR or cameras. Additionally, it is possible to use multiple costmaps from various sensors of the same type, such as several cameras in different positions, thereby strengthening the perception system.

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.95\columnwidth]{src/Integración RealSense SDV/imgs_D435I/costmap_multilayer.png}
    \caption{The Multilayer Costmap concept~\cite{costmap_multilayer}.}\label{fig:costmap_multilayer}
\end{figure}

\subsection{Optical Properties of the RGB-D Camera}\label{sec:rgb_d_properties}

    \subsubsection*{Field of View}
    The field of view (FOV) of a camera allows us to understand the extent of the observable scene in an image or video. It represents the angular range that the camera lens can capture. It is generally defined in both horizontal and vertical dimensions. The horizontal field of view determines the left-to-right range, while the vertical field of view covers the up-and-down range. Spatially, the FOV is described by a frustum, which is a geometric shape that plays a crucial role in understanding and visualizing the camera's field of view (see fig.~\ref{fig:frustum}). The frustum defines the volume of space that the camera can capture in a scene and is essentially a truncated pyramid, where the apex of the pyramid is at the camera lens, and the base of the pyramid represents the image plane or sensor.

    \begin{figure}[htbp]
        \centering
        \includegraphics[width=6cm]{src/Integración RealSense SDV/imgs_D435I/frustum.png}
        \caption{Three-dimensional representation of a camera's field of view~\cite{frustum}.}\label{fig:frustum}
    \end{figure}

    The camera's frustum is defined by three parameters: the near and far clipping planes, the horizontal and vertical fields of view, and the aspect ratio of the image. The near and far clipping planes represent the minimum and maximum distances from the camera at which objects will be in focus and included in the captured image. The shape of the frustum is determined by extending lines from the camera lens through the corners of the near and far clipping planes (see fig. \ref{fig:frustum}). Similarly, the values of the horizontal and vertical FOV (\textit{fovy} in fig. \ref{fig:frustum_fov}), often specified in degrees or radians, indicate the angular extent covered by the lens. Furthermore, the aspect ratio of the image, which represents the proportional relationship between width and height, influences how the FOV is distributed (see fig. \ref{fig:frustum_fov}).

    \begin{figure}[htbp]
        \centering
        \includegraphics[width=\columnwidth]{src/Integración RealSense SDV/imgs_D435I/frustum_FOV.png}
        \caption{Characteristic parameters of a camera's field of view\cite{frustumfov}.}\label{fig:frustum_fov}
    \end{figure}

    \subsubsection*{Depth Map}
    The depth map or point cloud is a three-dimensional representation of the environment captured by a depth camera. In this context, depth is measured as the distance from the camera to objects in the scene. The point cloud consists of a set of coordinates ($x, y, z$), where each point represents the spatial position of a detected object in the image captured by the camera.\\
    This type of three-dimensional information is fundamental for perception and autonomous navigation applications in robotics. In the context of ROS, the autonomous navigation stack uses the point cloud to build and update occupancy maps of the robot's environment. These maps are used to plan safe routes and avoid obstacles during autonomous navigation. This type of data is represented using the PointCloud2 message from the ROS framework~\cite{pointCloud2_ros_msg}. The message' structure contains detailed information about the point cloud, including the three-dimensional coordinates of each point, as well as additional information such as data on color and signal intensity.


==> src/Autores.tex <==
\label{sec:autores}
%\author{
%    \IEEEauthorblockN{Jhair S. Gallego and Ricardo E. Ramirez} \\
%    \IEEEauthorblockA{
%        \textit{Department of Mechanical and Mechatronics Engineering}\\
%        \textit{Universidad Nacional de Colombia}\\
%         \\
%        \{jhgallego, reramirezh\}@unal.edu.co
%        }
%}

\author{\IEEEauthorblockN{1\textsuperscript{st} Jhair S. Gallego}
\IEEEauthorblockA{\textit{Department of Mechanical and Mechatronics Engineering} \\
\textit{Universidad Nacional de Colombia}\\
Bogotá, Colombia \\
jhgallego@unal.edu.co}
\and
\IEEEauthorblockN{2\textsuperscript{nd} Ricardo E. Ramirez}
\IEEEauthorblockA{\textit{Department of Mechanical and Mechatronics Engineering} \\
\textit{Universidad Nacional de Colombia}\\
Bogotá, Colombia \\
reramirezh@unal.edu.co}}

==> src/Conclusiones.tex <==
\section{Conclusions}\label{sec:conclusiones}
\begin{itemize}

    \item The integration of the RGB-D camera significantly improves the autonomous vehicle's ability to identify and avoid obstacles, especially those not visible by the LiDAR. This provides robustness in trajectory planning in dynamic environments.
    
    %\item The work addresses previous issues of reliability in motor communication and the limited detection of lateral obstacles. The implementation of the RGB-D camera and the adjustment of costmap parameters, such as the minimum and maximum height of obstacles, reduces detection errors and improves the operational autonomy of the SDV.
    
    \item The use of technologies like Docker to standardize the development environment and ensure experiment replicability is a key point of this work. This allows for efficient integration and testing of new cameras and algorithms, facilitating the maintenance and expansion of the autonomous navigation system in the future.
    
    \item The integration of the depth camera opens opportunities for the development of new algorithms based on machine vision, which can enhance the vehicle's operational capabilities, such as implementing decision trees based on object identification.
    
\end{itemize}

\section{Future work}
Filtering depth points by adjusting the camera's frustum parameters is a simplistic approach. The multilayer costmap can be enhanced by using more sophisticated algorithms, such as density-based point cloud filtering. The current method fails to identify and filter out some single-point data generated either because of camera's noise, or when facing reflective surfaces such as glass. Implementing a density-based filter could potentially mitigate this issue, taking into account that objects have a high point cloud density as can be seen in figure~\ref{fig:costmap_pointcloud_ranges}.

==> src/Implementacion/D435i_nav_stack_integration.tex <==
%Parameters modified in .yaml files
As mentioned in sections~\ref{sec:nodos_nav_stack} and~\ref{sec:costmap}, integrating a new sensor requires adjusting certain configuration parameters in the navigation system. In Figure~\ref{fig:costmap_pointcloud_ranges}, it can be observed that as the viewing plane of the camera's frustum extends further, the points exhibit greater dispersion and fail to accurately represent objects at those distances, such as walls in this case. Consequently, the costmap generates a false positive for an obstacle (represented in purple), which impacts trajectory planning for target points intersecting the affected areas. Therefore, the detection range of points as obstacles is limited to a frontal distance of less than $2m$ and a height range between $0.35m$ and $1.0m$. Table~\ref{table:costmap_params} provides a summary of these and other relevant configuration parameters. These define a frustum as described in section~\ref{sec:rgb_d_properties} and the ROS topic's name and data type to which the point cloud information comes from. The functionality of each parameter can be referenced from the official documentation of the /move\_base package~\cite{costmap_2d_parameters}.

\begin{figure}[htbp]
    \centering
    \includegraphics[width=\columnwidth]{src/Implementación/imgs/costmap_pointcloud_ranges.png}
    \caption{False positive clasification of obstacles when using default detection range limits in \textit{costmap\_2d} parameters.}\label{fig:costmap_pointcloud_ranges}
\end{figure}

\begin{table}[htbp]
    \centering
    \caption{Camera integration parameters for costmap}
    \begin{tabular}{|c|c|}
        \hline
        \textbf{data\_type} & PointCloud2  \\
        \hline
        \textbf{topic} & camera/depth/color/points \\
        \hline
        \textbf{marking} & true \\
        \hline
        \textbf{clearing} & true \\
        \hline
        \textbf{max\_obstacle\_height} & 1.0 \\
        \hline
        \textbf{min\_obstacle\_height} & 0.35 \\
        \hline
        \textbf{obstacle\_range} & 2.0 \\
        \hline
        \textbf{raytrace\_range} & 2.0  \\
        \hline
    \end{tabular}
    \label{table:costmap_params}
\end{table}


==> src/Implementacion/Entorno_de_desarrollo.tex <==
%\subsection{Development Environment}
To avoid overloading the operating system on the NUC when running graphical applications on Linux, the distributed architecture of ROS is used under a client-server model (see fig.~\ref{fig:cliente_servidor}). In this way, the NUC can operate without a graphical interface (\textit{headless} mode), and the data published by the topics are consulted over the Wi-Fi network. Visualization and data analysis applications run on a client, a computer connected to the same network, leveraging the resources of both devices. As shown in fig. \ref{fig:rviz_costmap_view}, using the Rviz visualizer from an external computer, we can observe sensors' readings and how it is interpreted by the vehicle. This method facilitates the troubleshooting process and effectively monitors the vehicle's status in real-time. Additionally, this architecture allows multiple clients to query the vehicle's data, improving the scalability of the development environment.

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.95\columnwidth]{src/Arquitectura/imgs/cliente_servidor.png}
    \caption{Client-server architecture.}\label{fig:cliente_servidor}
\end{figure}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.7\columnwidth]{src/Arquitectura/imgs/rviz_costmap_view.png}
    \caption{Perception of the surrounding world by the SDV.}\label{fig:rviz_costmap_view}
\end{figure}

\subsection*{Docker Technology}

To ensure consistency in software versions across different clients and to guarantee the replicability of the development environment, Docker is used. This technology allows the creation of a container defined in a plain text file, commonly called a Dockerfile, which (for the purposes of this work) unifies the use of Rviz, Gazebo, and ROS (Noetic) in a standardized environment, facilitating the replication of the development environment on any client.


==> src/Implementacion/Implementaci__n.tex <==
\section{Implementation}

\subsection{\textbf{Development Environment}}
\input{src/Implementación/Entorno_de_desarrollo.tex}

\subsection{\textbf{Intel RealSense D435i Depth Camera}}
\input{src/Implementación/Use_of_D435i.tex}

\subsection{\textbf{Integration with the Navigation System}}
\input{src/Implementación/D435i_nav_stack_integration.tex}


==> src/Implementacion/R200_troubleshooting.tex <==
%\subsubsection{Configuración en ROS de Cámara RealSense R200}\\
    % Problemas del puerto, desincronización, muestra de la nube de puntos
    % Lo anterior como justificación del cambio de cámara y muestra de la nube de puntos con la D435i.
    Conforme la hoja técnica del fabricante~\cite{r200_intel_sdk}, para utilizar la cámara R200 es necesario contar con requerimientos de sistema específicos, los cuales, según lo detallado en la sección~\ref{sec:vehiculo_de_trabajo}, se  satisfacen correctamente.

    \begin{itemize}
        \item \textbf{Versión Kernel sistema operativo:} Bajo el sistema operativo Linux, se debe contar con versiones de Kernel 4.4.x o 5.5 (el más actual a 2023 es la versión 6.5). 
        \item \textbf{Puerto USB 3.0:} Es necesario que la cámara sea conectada o alimentada por medio de un puerto USB 3.0 SuperSpeed, debido a la tecnología de driver de video que maneja (UVCVIDEO).
    \end{itemize}

    Se realiza la lectura de los datos provistos por la cámara por medio de ROS y se visualizan las imágenes bajo los distintos formatos que esta genera. En la figura \ref{fig:r200_depth_samples} se observan (en la parte superior) las imágenes de profundidad tipo \textit{depth\_image} de los lentes izquierdo y derecho de la cámara (conforme fig.~\ref{fig:r200_parts}). Del mismo modo, en la figura \ref*{fig:r200_point_cloud_sample}, la nube de puntos tridimentsional, generada a partir de la combinación de los datos de las imágenes obtenidas en cada uno de los lentes, conforme la teoría de visión~\cite{depth_calculation_rgbd}. Del mismo modo, en la figura \ref{fig:r200_stereo_sample} se observan las imágenes obtenidas por la cámara stereo de la Intel R200 (conforme fig. ~\ref{fig:r200_parts}).
    
    \begin{figure}[htpb]
        \centering
        
        \begin{subfigure}{0.5\columnwidth}
            \centering
            \includegraphics[width=0.9\linewidth]{src/Integración RealSense SDV/imgs/r200_left_lense_sample.png}
            \caption{Lente izquierdo}
            \label{fig:r200_left_lense_sample}
        \end{subfigure}%
        \begin{subfigure}{0.5\columnwidth}
            \centering
            \includegraphics[width=0.9\linewidth]{src/Integración RealSense SDV/imgs/r200_right_lense_sample.png}
            \caption{Lente derecho}
            \label{fig:r200_right_lense_sample}
        \end{subfigure}
        \hfill
        \begin{subfigure}{0.5\columnwidth}
            \centering
            \includegraphics[width=\linewidth]{src/Integración RealSense SDV/imgs/r200_point_cloud_sample.png}
            \caption{Mapa de profundidad generado}
            \label{fig:r200_point_cloud_sample}
        \end{subfigure}
    
        \caption{}
        \label{fig:r200_depth_samples}
    \end{figure}
    
    \begin{figure}[htbp]
        \centering
        \includegraphics[width=6cm]{src/Integración RealSense SDV/imgs/r200_stereo_sample.png}
        \caption{Visualización imágenes obtenidas con la cámara stereo IntelRealSense R200 en el LabFabEx}\label{fig:r200_stereo_sample}
    \end{figure}

    Con lo anterior, se corrobora el correcto funcionamiento de todos los lentes y sensores infrarojos de la cámara R200.


    \subsection*{Visualización en tiempo real} Se observó que la visualización en tiempo real (bajo la arquitectura presentada en \ref{sec:system_architecture}) de las imágenes provistas por la cámara está limitada por el ancho de banda de la red de internet que se utiliza. La frecuencia de actualización de lectura de imágenes desde un computador (distinto a la NUC) en la misma red LabFabEx es de 1Mb/s y el peso promedio de las imágenes de la cámara es de 1.1Mb, resultando (como se observa en la figura \ref*{fig:bandwidth}) en una frecuencia de recepción y por ende , de visualización de las imágenes, menor a 1Hz. Allí mismo se muestra que la frecuencia real de publicación de datos es de 60Hz, cuando es consultada directamente desde la NUC.

    \begin{figure}[htbp]
        \centering
        \includegraphics[width=6cm]{src/Integración RealSense SDV/imgs/bandwidth.png}
        \caption{Frecuencia de recepción de datos de imágen sobre la red WiFi LabFabEx}\label{fig:bandwidth}
    \end{figure}

    \subsection*{Desincronización}
    Para poder visualizar correctamente las imágenes de la cámara utilizando Rviz, este debe poder leer dos tipos de datos en tiempo real provistos por la cámara. Estos son, la imágen propiamente y un tópico que publica la información de configuración de la cámara (publicado en /camera\_info). Debido a la limitante de red mencionada anteriormente, en el cliente (en donde corre Rviz) no era posible visualizar los datos, pues el tipo de dato /camera\_info es más de mil veces más pequeño comparado con una sola imágen. Por esto, al cliente llegaban muchos más datos de este tipo por cada uno de cámara que se recibía. Cómo cada mensaje tiene una marca temporal había una desincronización y no se podía visualizar las imágenes. En la figura \ref{fig:r200topic_desincronization} se observa el error mencionado.


    \begin{figure}[htbp]
        \centering
        \includegraphics[width=6cm]{src/Integración RealSense SDV/imgs/r200topic_desincronization.png}
        \caption{Desincronización de los tópicos de la cámara para su correcta visualización en RViz a través de una red WiFi.}\label{fig:r200topic_desincronization}
    \end{figure}

    %, cuya estructura de flujo de datos se muestra en la figura \ref{fig:ROSnode_topic_syncronizer}.
    Para solucionar lo anterior, se creó un nodo de ROS. Este nodo toma como entradas (se suscribe) a los tópicos /camera\_info y /camera/image/raw y los republica pero a frecuencias sincronizadas. Esto lo logra al publicar la /camera\_info solo cuando llega un nuevo tópico de tipo /camera/image/raw. De esta manera, si bien se reduce la frecuencia de publicación del tópico /camera\_info, la información de ambas partes se mantiene sincronizada y por ende es posible visualizarla en un cliente remoto.

    %\begin{figure}[htbp]
    %    \centering
    %    \includegraphics[width=6cm]{src/Integración RealSense SDV/imgs/}
    %    \caption{Arquitectura nodo sincronizador de tópicos de cámara sobre red WiFi.}\label{fig:ROSnode_topic_syncronizer}
    %\end{figure}

    \subsection{Reinicio del puerto USB3.0}\\

    En la implementación, la lectura de imágenes por parte de la cámara no resulta estable cuando se utilizaba en conjunto con el \textit{stack} de navegación autónoma del SDV. Esto se evidencia en un reinicio del puerto USB 3.0 de la NUC, sin embargo, la comunicación no se reestablece sino hasta que se reinicia por completo la NUC, lo cual resulta inviable conforme los objetivos de operabilidad y autonomía del vehículo. El error se puede evidenciar por el texto \textit{uvcvideo: Failed to query (SET\_CUR) UVC control 1 on unit 7: -32 (exp. 2).} en la figura~\ref{fig:r200_usb30_port_reset}. La comunidad que da soporte a este tipo de cámaras relata que es un problema común con esta versión en específico, sin embargo, aún no se cuenta con una solución~\cite{github_issue_thread_r200_usb30_port_reset}.

        \begin{figure}[htbp]
        \centering
        \includegraphics[width=\columnwidth]{src/Integración RealSense SDV/imgs/r200_usb30_port_reset.png}
        \caption{Reset del puerto USB3.0}\label{fig:r200_usb30_port_reset}
    \end{figure}


==> src/Implementacion/Use_of_D435i.tex <==
%Justification for the change
As a RGB-D camera, the Intel D435i reference is used. This camera offers two main advantages: it can be connected via a USB 2.0 port and has long-term technological support from the manufacturer. For integration with ROS, the installation process recommended by the manufacturer was followed as in \cite{D435i_install_ros}. Figure~\ref{fig:d435i_point_cloud} illustrates the point cloud (in white) and the \textit{stereo} image generated by the camera.

\begin{figure}[htbp]
    \centering
    \includegraphics[width=\columnwidth]{src/Integración RealSense SDV/imgs_D435I/d435i_point_cloud.png}
    \caption{Point cloud generated by the D435i camera at LabFabEx.}\label{fig:d435i_point_cloud}
\end{figure}

\subsection*{Optical Properties of D435i}\label{sec:D435i_optical_caracteristics}

The technical specifications of the camera relevant to this work are summarized in Table~\ref{table:d435i_fov_specs}.

\begin{table}[htpb]
    \centering
    \caption{D435i FOV Specifications (adapted from \cite{D435i_specs}).}
    \begin{tabular}{|c|c|}
        \hline
        \textbf{Operating Range}        & 0.3m to 3m                       \\
        \hline
        \textbf{Field of View (FOV)}    & 87° (vertical) 58° (horizontal) \\
        \hline
        \textbf{Aspect Ratio}           & 16:9                            \\
        \hline
        \textbf{Depth Resolution}       & 1280 x 720                      \\
        \hline
    \end{tabular}
    \label{table:d435i_fov_specs}
\end{table}

% Section "RGB-D Camera"
\subsection*{Support Design for Mounting the Camera on the Vehicle}
The navigation system of the SDV requires knowing the \textit{pose} of the camera in order to perform the coordinate transformation to the central coordinate system of the SDV. This is achieved by providing the location of the camera's geometric center with respect to the central coordinate system (see fig.~\ref{fig:base_link_to_camera_link}). With this, it is possible to properly interpret and process the generated point cloud. Therefore, it is necessary to know the \textit{pose} of the camera to perform the corresponding transformation (see fig.~\ref{fig:base_link_to_camera_link}).

\begin{figure}[htpb]
    \centering
    
    \begin{subfigure}{0.5\columnwidth}
        \centering
        \includegraphics[width=0.9\linewidth]{src/Implementación/imgs/base_to_camera_tf_isometric.png}
        \caption{}
        \label{fig:base_to_camera_tf_isometric}
    \end{subfigure}%
    \begin{subfigure}{0.5\columnwidth}
        \centering
        \includegraphics[width=0.9\linewidth]{src/Implementación/imgs/base_to_camera_tf_lateral.png}
        \caption{}
        \label{fig:base_to_camera_tf_lateral}
    \end{subfigure}

    \caption{Relationship between the \textit{base\_link} and \textit{camera\_link} coordinate systems.}\label{fig:base_link_to_camera_link}
\end{figure}

Since it is not necessary for the camera to perform translations or rotations about its own axis, but rather to remain fixed, it is important that the position of the camera relative to the SDV base is always the same. To this end, a support was designed and manufactured to allow the camera to be directly coupled to a pre-existing mechanism on the SDV. This way, the position vector (and hence the coordinate system transformation) of the camera with respect to the base ($TF_{cb}$) can be obtained (see fig.~\ref{fig:base_link_to_camera_link}). The position of the \textit{camera\_link} coordinate system relative to the \textit{base\_link} coordinate system is described by the vector~\ref{eq:tf_cb_vector}:

\begin{equation}
    \mathbf{TF}_{cb} = \langle 0.345, 0, 0.28 \rangle m \label{eq:tf_cb_vector}
\end{equation}

The final design is shown in fig.~\ref{fig:camera_support}, and the integration with the pre-existing mechanism along with the mounting of the camera is shown in fig.~\ref{fig:mechanism_and_camera_support}. 

\begin{figure}[htpb]
    \centering
    
    \begin{subfigure}{0.5\columnwidth}
        \centering
        \includegraphics[width=0.8\linewidth]{src/Implementación/imgs/soporte_superior.png}
        \caption{}
        \label{fig:}
    \end{subfigure}%
    \begin{subfigure}{0.5\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{src/Implementación/imgs/soporte_lateral.png}
        \caption{}
        \label{fig:}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.5\columnwidth}
        \centering
        \includegraphics[width=0.8\linewidth]{src/Implementación/imgs/soporte_isométrico.png}
        \caption{}
        \label{fig:}
    \end{subfigure}%
    \begin{subfigure}{0.5\columnwidth}
        \centering
        \includegraphics[width=\linewidth]{src/Implementación/imgs/camera_support.png}
        \caption{}
        \label{fig:camera_support}
    \end{subfigure}
    
    \caption{D435i camera support. \textit{(a), (b), (c)}: Camera support mounted on mechanism. \textit{(d)}: Isometric view of support's CAD model.}
    \label{fig:mechanism_and_camera_support}
\end{figure}



==> src/Integracion_RealSense_SDV/D435I.tex <==
\section{Uso cámara Intel RealSense D435i}

Debido a la limitante de poder utilizar la cámara en simultáneo con el \textit{stack} de navegación autónoma del SDV por los problemas energéticos relacionados con el puerto USB3.0 anteriormente mencionados, se cambió la cámara de profundidad a la referencia D435i de la misma casa matriz. Esta cámara presenta la misma prestaciones que la anterior, sin embargo, ese posible utilizarla por medio de un puerto USB2.0. Además que cuenta con soporte tecnológico a largo plazo \cite{D435i_specs}.\\

Se siguió el proceso de instalación recomendado por el fabricante en \cite{D435i_install_ros}. Debido al entorno Dockerizado que se construyó inicialmente, la integración de esta nueva cámara al código ya realizado resultó ventajoso, demostrando así el beneficio de utilizar tecnologías que faciliten la replicabilidad y modularización de los desarrollos a base de código. \\


\subsubsection{Uso de la nube de puntos para la evasión de obstáculos}

Debido a las limitaciones que presentó el enfoque de simular un disposito LiDAR a través de la cámara, se propone ahora utilizar el campo de visión completo de la misma, al hacer uso del mapa de profundidad generado por la cámara.

\subsubsection{Ángulo de visión de la cámara}
Comprender el campo de visión (FOV por sus siglas en inglés) de una cámara es crucial para comprender la extensión de la escena observable en una imagen o vídeo. El FOV representa el rango angular que puede capturar la lente de la cámara. Por lo general, se define en dimensiones tanto horizontales como verticales. El campo de visión horizontal determina el intervalo de izquierda a derecha, mientras que el campo de visión vertical cubre el rango de arriba a abajo. \\

Espacialmente, el FOV se describe por medio de un tronco trapezoidal o frustum (por su nombre en inglés) \cite{frustum_wikipedia} el cual es una forma geométrica que desempeña un papel crucial para entender y visualizar el campo de visión (FOV) de una cámara. El frustum es esencialmente una pirámide truncada, donde el ápice de la pirámide se encuentra en la lente de la cámara, y la base de la pirámide representa el plano de la imagen o el sensor. El frustum define el volumen del espacio que la cámara puede "ver" o capturar en una escena (ver figura \ref{fig:frustum})

\begin{figure}[htbp]
    \centering
    \includegraphics[width=6cm]{src/Integración RealSense SDV/imgs_D435I/frustum.png}
    \caption{Representación tridimensional del ángulo de visión de una cámara (tomado de \cite{frustum}).}\label{fig:frustum}
\end{figure}

El frustum de la cámara se define mediante seis parámetros: la distancia focal de la cámara, las dimensiones del plano de la imagen o del sensor, y los planos de recorte cercano y lejano. Los planos de recorte cercano y lejano representan las distancias mínima y máxima desde la cámara en las que los objetos estarán enfocados e incluidos en la imagen capturada. La forma del frustum se determina mediante la extensión de líneas desde la lente de la cámara a través de las esquinas de los planos de recorte cercano y lejano (ver figura \ref{fig:frustum}). Del mismo modo, los valores de FOV horizontal y vertical (\textit{fovy} en fig. \ref{fig:frustum_fov}), a menudo especificados en grados o radianes, indican la extensión angular cubierta por la lente. Además, la relación de aspecto de la imagen, que representa la relación proporcional entre el ancho y el alto, influye en cómo se distribuye el FOV (ver fig. \ref{fig:frustum_fov}).

\begin{figure}[htbp]
    \centering
    \includegraphics[width=6cm]{src/Integración RealSense SDV/imgs_D435I/frustum_FOV.png}
    \caption{Parámetros característicos del ángulo de visión de una cámara (tomado de \cite{frustumfov}).}\label{fig:frustum_fov}
\end{figure}

Las especificaciones técnicas de la cámara con lo que al ángulo de visión respecta, provistas por el fabricante \cite{D435i_specs}, son las siguientes

\begin{table}
    \centering
    \begin{tabular}{|c|c|}
        \hline
        \textbf{Rango de Operación}        & 0.3m a 3m                       \\
        \hline
        \textbf{Ángulo de Visión (FOV)}    & 87° (vertical) 58° (horizontal) \\
        \hline
        \textbf{Relación de Aspecto}       & 16:9                            \\
        \hline
        \textbf{Resolución de Profundidad} & 1280 x 720                      \\
        \hline
    \end{tabular}
    \caption{Especificaciones FOV D435i (tomado de \cite{D435i_specs}).}
    \label{tab:d435i_fov_specs}
\end{table}


\subsubsection{Qué es el mapa de profundidad}
El mapa de profundidad o nube de puntos (point cloud) generado por una cámara como la Intel RealSense es una representación tridimensional del entorno capturado por la cámara. En este contexto, la profundidad se mide como la distancia desde la cámara hasta los objetos en la escena. La nube de puntos consiste en un conjunto de coordenadas tridimensionales (x, y, z), donde cada punto representa la posición espacial de un objeto detectado en la imagen capturada por la cámara. \\

Este tipo de información tridimensional es fundamental para aplicaciones de percepción y navegación autónoma en robótica. En el contexto de ROS (Robot Operating System), el stack de navegación autónoma utiliza la nube de puntos generada por la cámara para construir y actualizar mapas de ocupación del entorno del robot. Estos mapas se utilizan para planificar rutas seguras y evitar obstáculos durante la navegación autónoma. \\

En cuanto a la estructura técnica del mensaje del tópico que publica la cámara con este mapa de profundidad, comúnmente se utiliza el mensaje PointCloud2 de ROS. Este mensaje contiene información detallada sobre la nube de puntos, incluyendo las coordenadas tridimensionales de cada punto, así como información adicional como intensidades de color y datos de intensidad de señal en el caso de cámaras RGB-D. \\

En resumen, el mapa de profundidad generado por cámaras como la Intel RealSense proporciona datos tridimensionales cruciales para la navegación autónoma en robótica, y la representación de este mapa se realiza comúnmente a través del mensaje PointCloud2 en el entorno de ROS. En la figura \ref*{fig:d435i_point_cloud} se obseva un ejemplo de la nube de puntos generada por la cámara en el LabFabEx y visualizada con la herramienta RViz.

\begin{figure}[htbp]
    \centering
    \includegraphics[width=8cm]{src/Integración RealSense SDV/imgs_D435I/d435i_point_cloud.png}
    \caption{Nube de puntos generada por la cámara D435i en el LabFabEx }\label{fig:d435i_point_cloud}
\end{figure}

\subsubsection{Estructura de datos mensaje PointCloud2}
El mensaje \texttt{PointCloud2} en ROS es un tipo de mensaje utilizado para representar nubes de puntos en entornos tridimensionales. Este mensaje puede contener información sobre las coordenadas tridimensionales de los puntos, así como otros datos adicionales como colores, intensidades y campos personalizados. A continuación, te proporciono una descripción de la estructura típica del mensaje \texttt{PointCloud2}:

La estructura del mensaje \texttt{PointCloud2} está definida por varios campos:

\textbf{Header:}
\begin{itemize}
    \item Contiene información de temporización y secuencia para sincronización con otros mensajes en ROS.
\end{itemize}

\textbf{Height y Width:}
\begin{itemize}
    \item \texttt{height} y \texttt{width} indican las dimensiones de la matriz de puntos. Para nubes de puntos, \texttt{height} suele ser 1, y \texttt{width} es el número total de puntos.
\end{itemize}

\textbf{Fields:}
\begin{itemize}
    \item Este campo describe la información contenida en cada punto de la nube. Cada elemento en el array \texttt{fields} especifica el nombre del campo, el tipo de dato (por ejemplo, "float32" para coordenadas), y el desplazamiento en bytes dentro de la estructura de datos.
\end{itemize}

\textbf{Is\_bigendian y Point\_Step:}
\begin{itemize}
    \item \texttt{is\_bigendian} indica si el formato de datos es big-endian o little-endian.
    \item \texttt{point\_step} es el número total de bytes en un punto.
\end{itemize}

\textbf{Row\_Step:}
\begin{itemize}
    \item Especifica la cantidad de bytes en una fila completa de puntos (útil si los puntos no están continuos en la memoria).
\end{itemize}

\textbf{Data:}
\begin{itemize}
    \item Contiene los datos de la nube de puntos como una secuencia de bytes. Los datos se organizan según la información proporcionada en los campos anteriores.
\end{itemize}

\subsubsection{Matriz de ocupación: concepto de cómo funciona en ROS}
El sistema de navegación autónoma en ROS utiliza mapas de costos o costmaps por su nombre en inglés para representar la información sobre la ocupación del entorno y facilitar la toma de decisiones de planificación del robot. En el contexto del stack de navegación autónoma de ROS, hay dos niveles principales de mapas de costo: el \textit{\textbf{global\_costmap}} y el \textit{\textbf{local\_costmap}}. Ambos mapas trabajan en conjunto para permitir la navegación segura del robot en su entorno. En la figura \ref{fig:move_base_arq} se observa cómo se integran y comunican estos dos componentes dentro del \textit{stack} de navegación autónoma del SDV.\\

\begin{figure}[htbp]
    \centering
    \includegraphics[width=8cm]{src/Integración RealSense SDV/imgs_D435I/move_base_arq.png}
    \caption{Ubicación del mapa de costos dentro del stack de navegación autónoma del SDV (tomado y adaptadode \cite[text]{move_base_ros_node}).}\label{fig:move_base_arq}
\end{figure}

\begin{itemize}
    \item Global Costmap:
          El global\_costmap tiene como objetivo proporcionar una representación de alto nivel del entorno y se utiliza para la planificación global de rutas. Este costmap se genera a partir de información estática y dinámica. La información estática generalmente proviene de mapas estáticos proporcionados de antemano, mientras que la información dinámica proviene de sensores en tiempo real, como láseres o cámaras.

    \item Local Costmap:
          El local\_costmap opera a un nivel más detallado y se utiliza para la navegación local y la evasión de obstáculos cercanos. Este costmap se actualiza más frecuentemente y utiliza información de sensores en tiempo real, como láseres y cámaras.

    \item Matriz de Ocupación:
          La representación principal del entorno en el mapa de costos global y local es una matriz de ocupación. En esta matriz, cada celda representa una región del entorno y tiene un valor que indica el nivel de ocupación. Comúnmente, se utiliza una escala de valores discretos, como: 0 (celda libre); Indicando que la celda está libre y no obstaculizada o 100 (celda ocupada);Indicando que la celda está ocupada por un obstáculo.
          \textbf{El SDV utiliza esta matriz para planificar rutas seguras a través del entorno.}

\end{itemize}

\textbf{Costmap Multicapa:}
La superposición de los mapas de costo global y local permite obtener una representación más completa y detallada del entorno y es conocida como costmap multicapa. Esta matriz tiene en cuenta tanto la información global como la local. En la figura \ref{fig:costmap_multilayer} se observa una representación conceptual del mapa de costos.

\begin{figure}[htbp]
    \centering
    \includegraphics[width=8cm]{src/Integración RealSense SDV/imgs_D435I/costmap_multilayer.png}
    \caption{Mapa de costos. Tomado de~\cite{costmap_multilayer}}\label{fig:costmap_multilayer}
\end{figure}

\subsubsection{Integración con ROS (fine tunning)}
- cómo la inclinación de la cámara afecta el mapa de costos (altura mínima tomada en cuenta)
- distancia máxima tomada en cuenta

\subsubsection{Pruebas de funcionamiento}
- Video-prueba con el "puente de plástico"




==> src/Integracion_RealSense_SDV/Integracion_RealSense_SDV.tex <==
\section{Integración ZED con ROS}

\subsection{Motivación}
La destreza en la evasión de obstáculos del SDV puede mejorarse y fortalecerse mediante la incorporación de una cámara de profundidad a su equipo tecnológico. La integración y configuración de este dispositivo al código preexistente del vehículo no solo pueden mejorar su autonomía operativa para la evasión de obstáculos, sino que también proporciona una plataforma versátil para futuras aplicaciones basadas en visión de máquina.

\subsection{Propuesta}
La propuesta consiste en la transformación de los datos provenientes de la cámara a un formato de datos compatible con LIDAR, con el objetivo de simular la integración de un LIDAR dentro del stack de navegación autónoma. Para ilustrar este proceso, se presenta una imagen representativa que visualiza la interacción entre los diferentes tipos de datos, específicamente los mensajes de ROS que se utilizan en esta simulación. Este enfoque permitirá evaluar y mejorar la eficacia del sistema de navegación autónoma al considerar la información proporcionada tanto por la cámara como por el LIDAR simulado.
%\textbf{La idea es convertir los datos de la cámara a un tipo de dato lidar. De tal modo que se simule la adición de un lidar al stack de navegación autónoma. (Se muestra una imágen representativa que muestre los tipos de datos (mensajes de ros que interactuan))}

\subsection{Entorno de desarrollo}

%\textbf{Aquí se muestra el entorno que se utilizó. Una imágen docker en mi computador para poder leer los tópicos del SDV.}
Se presenta el entorno utilizado en el que se despliega una imagen Docker en un computador cliente. Esta configuración específica se implementa para facilitar la lectura de los tópicos del Sistema de Vehículo Autónomo (SDV). La utilización de una imagen Docker permite una gestión eficiente y aislada de los componentes del entorno, garantizando así un acceso y análisis efectivo de los datos generados por el SDV.

\subsection{Paquete \textit{depthImage2LaserScan}}

La solución propuesta consiste en la implementación de un paquete de ROS llamado \textit{depthImage2LaserScan}, el cual permite la conversión de una imágen de profundidad (generada por una cámara de RGB-D) a un tipo de dato \textit{laserScan}. Esto se realiza de tal modo que pueda existir una integración simple con el tipo de datos que ya maneja el código base de los SDV. A saber, \textit{laserScan} generado por un dispositivo con tecnología LiDAR.

En la figura \ref{fig:arquitecture} se muestra la arquitectura de solución propuesta. En donde el recuadro resaltado en rojo representa el nodo a implementar, las flechas que apuntan desde y hacia este, representan el tipo de dato intercambiado y los recuadros no resaltados, representan nodos ya integrados sobre el código fuente del SDV.

\begin{figure}[htbp]
    \centering
    \includegraphics[width=6cm]{src/Integración RealSense SDV/imgs/arquitecture.png}
    \caption{}\label{fig:arquitecture}
\end{figure}

\subsection{Recursos tecnológicos utilizados}

\begin{itemize}
    \item \textbf{Computación:} Se trabaja con el SDV versión 3 del Laboratorio de Fábrica Experimental (LabFabEx), el cual cuenta con un computador NUC de Intel.~\cite{NUC_intel_webpage}

    \item \textbf{Cámara:} Se utiliza la cámara RGB-D Intel RealSense R200~\cite{r200_datasheet}
\end{itemize}

\subsection{Implementación}

La implementación consiste en instalar el paquete \textit{depthImage2LaserScan}~\cite{depthImage2LaserScan_ros_wiki} provisto por la comunidad de código abierto de ROS.

\subsubsection{Configuracón en ROS de Cámara RealSense}:

Para utilizar la cámara R200 es necesario contar con requerimientos de sistema específicos~\cite{r200_datasheet}.

\begin{itemize}
    \item \textbf{Versión Kernel sistema operativo:} La cámara solo se puede utilizar con un kernel específico de linux (4.4.x y 5.5) el más actual es 6.5 (2023).
    \item \textbf{Puerto USB 3.0:} Es necesario que la cámara sea conectada o alimentada por medio de un puerto USB 3.0 SuperSpeed, debido a la tecnología de driver de video que maneja (UVCVIDEO).
\end{itemize}

Si bien el SDV cumple con los requerimientos anteriormente mencionados, en la implementación, la lectura de imágenes por parte de la cámara no era estable cuando se utilizaba en conjunto con el \textit{stack} de navegación autónoma del SDV. Esta inestabilidad se representa en un reinicio de puerto USB3.0 de la NUC y posteriormente, la inhabilidad para establecer conexión con la cámara si no se realiza un reinicio completo de la NUC.\\

Fuera del problema anteriormente mencionado, la configuración del susodicho paquete de ROS resultó exitosa y se pudieron visualizar las imágenes obtenidas desde cámara bajo los distintos formatos que esta genera. En la figura \ref{fig:r200_images_sample} se observan (en la parte superior) las imágenes de profundidad tipo \textit{depth\_image} de los lentes izquierdo y derecho de la cámara. Asimismo, en la parte inferior, la nube de puntos tridimentsional, generada a partir de las imágenes anteriores. Del mismo modo, en la figura \ref{fig:r200_images_sample2} se observan las imágenes obtenidas por la cámara stereo de la Intel R200.

\begin{figure}[htbp]
    \centering
    \includegraphics[width=6cm]{src/Integración RealSense SDV/imgs/r200_images_sample.png}
    \caption{Visualización imágenes obtenidas con la cámara RGB-D IntelRealSense R200 en el LabFabEx}\label{fig:r200_images_sample}
\end{figure}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=6cm]{src/Integración RealSense SDV/imgs/r200_images_sample2.png}
    \caption{Visualización imágenes obtenidas con la cámara stereo IntelRealSense R200 en el LabFabEx}\label{fig:r200_images_sample2}
\end{figure}

\subsubsection[short]{Visualización en tiempo real:} Se observó que la visualización en tiempo real de las imágenes provistas por la cámara está limitada por el ancho de banda de la red de internet que se utiliza. La frecuencia de actualización de lectura de imágenes desde un computador (distinto a la NUC) en la misma red LabFabEx es de 1Mb/s y el peso promedio de las imágenes de la cámara es de 1.1Mb, resultando (como se observa en la figura \ref*{fig:bandwidth}) en una frecuencia de recepción y por ende , de visualización de las imágenes, menor a 1Hz. Allí mismo, se muestra que la frecuencia real de publicación de datos es de 60Hz.

\begin{figure}[htbp]
    \centering
    \includegraphics[width=6cm]{src/Integración RealSense SDV/imgs/bandwidth.png}
    \caption{Frecuencia de recepción de datos de imágen sobre la red WiFi LabFabEx}\label{fig:bandwidth}
\end{figure}

\subsection{Desincronización}
Teniendo en cuenta que para que Rviz pueda visualizar adecuadamente las imágenes de la cámara, este debe contar con dos tipos de datos en tiempo real provistos por la cámara. Estos son, la imágen como tal y un tópico que publica la información de configuración de la cámara (publicado en /camera\_info). Debido a la limitante de red mencionada anteriormente en el cliente (en donde corre Rviz) no era posible visualizar los datos, pues el tipo de dato /camera\_info es más de mil veces más pequeño comparado con una sola imágen. Por esto, al cliente llegaban muchos más datos de este tipo por cada uno de cámara. Cómo cada mensaje tiene una marca temporal había una desincronización y no se podía visualizar las imágenes. En la figura \ref{fig:r200topic_desincronization} se observa el error mencionado.


\begin{figure}[htbp]
    \centering
    \includegraphics[width=6cm]{src/Integración RealSense SDV/imgs/r200topic_desincronization.png}
    \caption{Desincronización de los tópicos de la cámara para su correcta visualización en RViz a través de una red WiFi.}\label{fig:r200topic_desincronization}
\end{figure}


Para solucionar lo anterior, se creó un nodo de ROS, cuya estructura de flujo de datos se muestra en la figura \ref{fig:ROSnode_topic_syncronizer}. Este nodo toma como entradas (se suscribe) a los tópicos /camera\_info y /camera/image/raw y los republica pero a frecuencias sincronizadas. Esto lo logra al publicar la /camera\_info solo cuando llega un nuevo tópico de tipo /camera/image/raw. De esta manera, si bien se reduce la frecuencia de publicación del tópico /camera\_info, la información de ambas partes de mantiene sincronizada y por ende es posible visualizarla en un cliente remoto.

\begin{figure}[htbp]
    \centering
    \includegraphics[width=6cm]{src/Integración RealSense SDV/imgs/}
    \caption{Arquitectura nodo sincronizador de tópicos de cámara sobre red WiFi.}\label{fig:ROSnode_topic_syncronizer}
\end{figure}


\subsection{Resultados integración RealSense R200}

Se realizó la integración al stack de navegación, permitiendo obtener datos desde la cámara y utilizarlos como datos generados por un LiDAr. Sin embargo, debido al limitado campo de visión de la cámara (que es menor a 180°) comparado con el de un LiDAR, la cantidad de información de distancias u objetos que esta le provee al algoritmo de navegación autónoma es insuficiente como para permitir que el SDV pueda navegar por sí solo con una alta confiabilidad. De las pruebas que se realizaron, en ninguna el SDV lograba encontrar y seguir una trayectoria de navegación.


\input{src/Integración RealSense SDV/D435I.tex}

==> src/Introduccion/Introducci__n.tex <==
\section{Introduction}

\subsection{Problem definition}

With the development of new technologies within the context of Industry 4.0, there is a push for intelligent and collaborative communication between robots in a factory. The main objective of this approach is for robots to be flexible in adapting their operations according to the changing demands of the factory. The implementation of collaborative robotics allows these agents to interact with one another, promoting flexibility in their operations. Adaptability in the manufacturing environment is not limited to robot interaction; it also addresses the need to adjust factory operations according to market dynamics. In a context where technologies are emerging rapidly and production needs are evolving, it is crucial for each robot to be flexible within the production chain. This flexibility facilitates an agile response to new demands without the need to incorporate new robots in every case.\\
The logistics of raw materials and manufactured items play a fundamental role in production processes. In the context of an experimental factory, there is an urgent need to transport items between the various machines that make up the facility. Self-Driving ground Vehicles (SDVs) enable the transportation of these items within production plants. These vehicles, upon receiving instructions from an external agent, plan trajectories and navigate autonomously, overcoming dynamic obstacles such as the presence of people or other robots.\\
The use of a 2D LiDAR sensor is common in the perception system of these vehicles. However, in certain scenarios, the effectiveness of trajectory execution is impacted due to the limited field of view provided by the sensor. The 2D LiDAR-based perception system cannot detect obstacles whose position or geometry lies outside the sensor's field of view. As shown in Figure \ref{fig:LiDAR_lateral_vertical_FOVs}, any obstacle whose geometry does not intersect with the red plane will affect the effective generation of trajectories that allow for evasion, as the perception system will not account for it, resulting in a collision. This generates operational failures in the production processes of the factories where the vehicles operate. To address this limitation, we propose the integration of a depth camera to the perception system of these vehicles, extending the field of view to three dimensions and accounting for new obstacle detection improvements. In this work, we describe the process of integration of a depth camera (RGB-D) into the navigation system of an SDV, we present a theoretical review of the concepts around this integration, describe the implementation of a multilayer occupancy grid, and evaluate its effectiveness in strengthening the obstacle detection process.

\begin{figure}[htpb]
    
    \centering
    \includegraphics[width=0.8\columnwidth]{src/Introducción/imgs/lidar_lateral_FOV_highlited_red.png}
    \caption{Vertical field of view concept for LiDAR 2D.}
    \label{fig:LiDAR_lateral_vertical_FOVs}
\end{figure}

\subsection{Working vehicle}\label{sec:vehiculo_de_trabajo}
For the development of this work, the SDV II~\cite{agv_2016_UAO} from the Experimental Factory Laboratory (LabFabEx) at the Universidad Nacional de Colombia was used. The vehicle is shown in Figure~\ref{fig:sdvII_unimedios}.

        \begin{figure}[htbp]
            \centering 
            \includegraphics[width=0.7\columnwidth]{src/Introducción/imgs/sdvII_unimedios.jpg}
            \caption{SDV II vehicle from the LabFabEx~\cite{sdvII_unimedios_report}.}\label{fig:sdvII_unimedios}
        \end{figure}

        This vehicle features a skid-steering kinematic architecture (see fig.~\ref{fig:skid-steering}), that allows it to move with two degrees of freedom. i.e., in the vehicle's local coordinate frame with origin in the geometric center of the vehicle, movement forward and backwards ($x$ direction) and rotations around the ground plane ($yaw$)~\cite{skid_steering_kinematics}. The vehicle's electronic components are classified as follows:

        \begin{enumerate}
            \item \textit{Computing and Navigation System:} Composed of an Intel NUC mini-computer with 8 GB of RAM, Two USB 2.0 ports, and one USB 3.0 port~\cite{NUC_intel_webpage}. The operating system used is Linux 18.04 (kernel v5.5), and navigation is implemented under the ROS Noetic framework~\cite{ros_noetic_docs}.
        
            \item \textit{Perception System:} Uses the 2D LiDAR sensor Sick-LMS102~\cite{sick_website}.
            
            \item \textit{Low-Level Control:} Uses a Tiva C Series board~\cite{tiva_datasheet}. It facilitates serial communication with the motor drivers responsible for the vehicle's propulsion.
    
    \end{enumerate}
    
    
    \begin{figure}[htbp]
        \centering
        \includegraphics[width=0.7\columnwidth]{src/Introducción/imgs/skid_steering_mechanism.png}
        \caption{Skid-steering architecture~\cite{skid_steering_diagram}.}\label{fig:skid-steering}
    \end{figure}


==> src/Introduccion/intro_v1.tex <==
%introducción separada por temas
Tema: Adaptabilidad de los robots:
    Texto: Con el desarrollo de nuevas tecnologías bajo el contexto de la industria 4.0 se busca la comunicación inteligente o colaborativa entre los robots de una fábrica, de tal modo que los robots sean flexibles en el ajuste de su operación conforme las necesidades que la fábrica demande. Del mismo modo, que estos opten por la comunicación con los demás agentes (robots) de su entorno logrando la flexibilidad a través de la robótica colaborativa.

    Tema: Adaptabilidad de la fábrica según el mercado:
    Texto: El mercado está cambiano constantemente y con el rápido emergimiento de nuevas tenologías y necesidades es necesario que las fábricas se puedan ajustar a las necesidades que se le demanden en donde cada robot que la conforma pueda ajustarse y ser flexible dentro de una cadena productiva de tal modo que pueda responder a las nuevas necesidades de producción de la fábrica sin necesidad de incluir nuevos robots en todos los casos.

    Tema: Logística del Transporte en cadenas de producción:
    Texto: Dentro de los procesos productivos un gran componente es la logística de la materia prima o los elementos fabricados, en donde se busca disponer de los materiales necesarios para realizar las tareas productivas. En una fábrica miniexperimental en donde surge la necesidad de transportar elementos entre las distintas máquinas que la conforman.

    Tema: Qué son los SDV
    Dentro de la necesidad del transporte de elementos, surgen los vehículos autónomos (SDV) que permiten el transporte automatizado entre diferentes lugares de las plantas de producción de manera autónoma, en donde un agente externo le indica a donde debe llegar y el robot debe planear y trayectoria y navegarla, evadiendo los obstáculos dinámicos que se le presenten en la trayectoria, como pueden ser personas u otros robots.

    Tema: El problema
    Texto1: El vehículo no se utiliza para ejecutar algún proceso puesto que no se sabe si este lo podrá ejecutar efectivamente, puesto que su fiabilidad operativa se intuye (porque no está cuantificada) es muy baja.
    Texto2: El vehículo no se utilizar en un proceso real porque no se conoce si qué tantas veces puede ejecutar satisfactoriament el proceso. Es decir, no se tiene confianza en la capacidad operativa del vehículo.


    Texto3: Para lograr un transporte autónomo efectivo, es preciso conocer la fiabilidad del mismo en su operación, tanto en la capacidad de navegar autónomamente en un entorno estático y dinámico, como en su capacidad para posicionarse de manera correcta en un lugar predeterminado. Es preciso contar con una alta fiablidad que permita determinar a qué tareas se puede someter el vehículo y ese responderá efectivamente. Además de proveer el contexto suficiente para que la fábrica pueda saber de qué manera o qué tanto debe adaptarse para integrar el vehículo con los demás agentes robóticos.


    %palabras clave:
    %-robótica colaborativa
    %-flexibilidad (que sean flexibles en su operación, tal que se puedan adaptar a las nuevas necesidades)
%
    %Texto redactado:
%
    %que el diseño del robot le permita ser flexible tal que se pueda adaptar a las nuevas necesidades pero tambien que
    %permita la comunicación con demás agentes de su entorno logrando la flexibilidad a través de la robótica colaborativa.
%

==> src/Resultados/Resultados.tex <==
\section{Results}

%\subsection{Verification of obstacle avoidance with the camera}
To verify that the camera is indeed assisting in trajectory planning by identifying objects, the following scenario was implemented. An obstacle in the form of a bridge, represented by plastic (hereafter referred to as \textit{the bridge}), was placed at a height of $60cm$, in such a way that it could not be detected by the LiDAR but could be identified by the camera, due to its vertical field of view (see fig.~\ref{fig:plastic_bridge_scenario}). The test consists of providing a target position to the vehicle, such that it initially generates a trajectory that should pass under the bridge.

\begin{figure}[htbp]
    \centering
    \includegraphics[width=\columnwidth]{src/Resultados/imgs/plastic_bridge_scenario.png}
    \caption{Testing scenario for obstacle avoidance with the RGB-D camera.}\label{fig:plastic_bridge_scenario}
\end{figure}

\begin{figure}[htpb]
    \centering

    \begin{subfigure}{\columnwidth}
        \centering
        \includegraphics[width=0.9\linewidth]{src/Resultados/imgs/(before) plastic_bridge_rviz_view.png}
        \caption{}
        \label{fig:before_plastic_bridge_rviz_view}
    \end{subfigure}
    \hfill
    \begin{subfigure}{\columnwidth}
        \centering
        \includegraphics[width=0.9\linewidth]{src/Resultados/imgs/(before) plastic_bridge_test_camera_view.png}
        \caption{}
        \label{fig:before_plastic_bridge_test_camera_view}
    \end{subfigure}

    \caption{Testing scenario before dynamic obstacle avoidance.}\label{fig:before_plastic_bridge_test}
\end{figure}

In figure~\ref{fig:before_plastic_bridge_test}, it can be seen that initially, a trajectory is generated so that the vehicle should go under the bridge. Once the camera identifies the obstacle, it is effectively projected onto the costmap, highlighted by a red box in figure~\ref{fig:after_plastic_bridge_test_rviz_view_highlighted}. Similarly, an alternative trajectory (green line) is recalculated to reach the proposed target location. In figure~\ref{fig:after_plastic_bridge_test_camera_view}, from the camera's perspective, both the bridge (obstacle) and its projection generated by the navigation system can be observed.

\begin{figure}[htpb]
    \centering
    \begin{subfigure}{\columnwidth}
        \centering
        \includegraphics[width=0.9\linewidth]{src/Resultados/imgs/(after) plastic_bridge_test_rviz_view(highlighted).png}
        \caption{}
        \label{fig:after_plastic_bridge_test_rviz_view_highlighted}
    \end{subfigure}
    \hfill
    \begin{subfigure}{\columnwidth}
        \centering
        \includegraphics[width=0.9\linewidth]{src/Resultados/imgs/(after) plastic_bridge_test_camera_view.png}
        \caption{}
        \label{fig:after_plastic_bridge_test_camera_view}
    \end{subfigure}

    \caption{Testing scenario after dynamic obstacle avoidance.}\label{fig:after_plastic_bridge_test}
\end{figure}


==> src/Resumen.tex <==
\begin{abstract}\label{sec:resumen}    
    This work describes the process of integrating a depth camera into the navigation system of a self-driving ground vehicle (SDV) and the implementation of a multilayer costmap that enhances the vehicle's obstacle identification process by expanding its two-dimensional field of view, based on 2D LIDAR, to a three-dimensional perception system using an RGB-D camera. This approach lays the foundation for a robust vision-based navigation and obstacle detection system. A theoretical review is presented and implementation results are discussed for future work.
\end{abstract}


\begin{IEEEkeywords}
    Occupancy grid, ROS, RGB-D depth camera, Docker, self-driving ground vehicle (SDV), obstacle avoidance.
\end{IEEEkeywords}

==> src/utils.tex <==
\begin{figure}[htbp]
    \centering
    \includegraphics[width=6cm]{}
    \caption{}\label{fig:}
\end{figure}

\begin{table}[htbp]
\centering
\begin{tabular}{|l|l|l|l|} 
\hline
 & S1 & S2 & S3  \\ 
\hline
a &    &    &     \\ 
\hline
b &    &    &     \\ 
\hline
c &    &    &     \\
\hline
\end{tabular}
\end{table}

% Importar pdfs completo "pages=-" o parcial "pages=2", etc
% \usepackage{pdfpages}
\newpage\hbox{}\thispagestyle{empty}\newpage
    \includepdf[pages=-,fitpaper]
    {Lab4/interrupcion_manejo_de_teclado.pdf}
